Jointly Learning Truth-Conditional Denotations and Groundings using Parallel Attention

We present a model that jointly learns the denotations of words together with their groundings using a truth-conditional semantics. Our model builds on the neurosymbolic approach of Mao et al. (2019), learning to ground objects in the CLEVR dataset (Johnson et al., 2017) using a novel parallel attention mechanism. The model achieves state of the art performance on visual question answering, learning to detect and ground objects with question performance as the only training signal. We also show that the model is able to learn flexible non-canonical groundings just by adjusting answers to questions in the training set.

==> model-scratch.tex <==
\subsubsection{Filter}
\begin{center}\ex{blue \textsf{X}}\end{center}

The \op{filter} operator filters a set of objects based on some
concept such as \conc{red} or \conc{cylinder}. It takes as
inputs (i) a specification of the concept (and corresponding
attribute such as \att{color} or \att{shape}); (ii) the vector of
objecthood parameters $h_i$ (iii) a vector $x \in [0,1]^n$ which
represents a fuzzy set capturing the results of earlier semantic
operators. Each component $x_i$ can be understood as the probability
that the object bound to grounding variable $v_i$ remains viable. When
no earlier semantic operators have been applied, the vector of
objecthoods $h_i$ is used; and (iv) 
the set of object grounding vectors $v_i$.

The \op{filter} operator first computes a matrix of representing the
degree to which each object fits each concept
$M \in \mathbb{R}^{|\mathcal{A}| \times n}$.

$$M_{[\conc{m},i]} = y_{\conc{m}} \cdot A_{\att{a}} v_i $$

Here $A_{\att{a}}$ is a linear transformation which moves the object
embedding $v_i$ into attribute space (e.g., \att{color}) and
$y_{\conc{m}}$ is a concept embedding for example $y_{\conc{red}}$.

We assume that concepts are mutually exclusive for a given object. To
capture this we perform a \textsc{softmax} operation on each column of
$M$. 

Finally, we take an elementwise \textsc{min} operation---representing
a fuzzy \textsc{and}---over (i) the row of $M$ representing the target
concept, (ii) the input viabilities $x_i$ and (iii) the objecthood
parameters $h_i$. This final \textsc{min} step represents the
composition of the results of this filter operation with earlier
semantic and object grounding operations.

\subsubsection{Relate}

\begin{center}\ex{\textsf{X} to the left of the blue cube}\end{center}

The \op{relate} operator computes the set of objects that stand in
some spatial relation with some target object. It takes as input (i)
the spatial relation (ii) a fuzzy set $\{x_i\}$ representing the
target object (iii) the set of object pair-embeddings
$\{ v_{ij}\}$ and (iv) the set of $\{h_i\}$ objecthood
parameters.

In the CLEVR database, all target objects in relations are definites
\ex{... to the left of \textbf{the cube}.} To capture the uniqueness
presupposition of definite noun phrases, we first renormalize the
target object vector so that it represents a probability distribution
over target objects $p = \textsc{renormalize}(x)$. \todo{is this correct?}

We next compute a matrix $O \in [0,1]^{n \times n}$ of probabilities
that each pair of objects stands in the relation.

$$O_{[i,j]} = \sigma((y_{\conc{m}} \cdot v_{ij}) \times z) $$

\noindent where $y_{\conc{m}}$ is a concept embedding for the relation
(e.g., $y_{\conc{behind}}$) and $z$ is a scaling parameter.

We then compute the joint probability that each object stands in the
relation with an another object  and that other object is the target
object as $t=Op$.

Finally, we take an elementwise \textsc{min} operation between each
value $t_i$ and the objecthood
parameters $h_i$.

\subsubsection{Relate Attribute Equality}

\begin{center}\ex{\textsf{X} that has the same color as the cube}\end{center}

The \op{relate-att-eq} operator computes the set of objects that
have the same concept value for some attribute as some target
object. It takes as input (i) the attribute (ii) a fuzzy set $\{x_i\}$
representing the target object (iii) the set of object groundings
$\{ v_{i}\}$ and (iv) the set of $\{h_i\}$ objecthood parameters.

As above, all target objects for attribute equality are
definites. Thus, we first renormalize the target object vector so that
it represents a probability distribution over target objects
$p = \textsc{renormalize}(x)$.

The \op{relate-att-eq} operator first computes a matrix representing the
degree to which each object fits each concept
$M \in \mathbb{R}^{|\mathcal{A}| \times n}$.

$$M_{[\conc{m},i]} = y_{\conc{m}} \cdot A_{\att{a}} v_i $$

Here, all variables are as in the \op{filter} operator.

We next compute a matrix $O \in [0,1]^{n \times n}$ of probabilities
that each pair of objects share a concept value.

$$O_{[i,j]} = e^{- \mathrm{KL(\textsc{softmax}(M_{[:,i]}) || \textsc{softmax}(M_{[:,j]}))}}$$
\noindent We assume here concept values are mutually exclusive for a particular
attribute (e.g., \conc{red} or \conc{blue} for \att{color}) by
applying \textsc{softmax} over each column of
$M$. We compute the probability that objects $i$ and
$j$ share a concept value by exponentiating the negative KL-divergence
between their concept distributions.

We then compute the joint probability that each object stands in the
relation with an another object  and that other object is the target
object as $t=Op$.

Finally, we take an elementwise \textsc{min} operation between each
value $t_i$ and the objecthood
parameters $h_i$.

\subsubsection{Query}

\begin{center}\ex{What's the color of the cube}\end{center}

The \op{query} operator computes the probability that a target object takes
on some value of an attribute. It takes as input (i) the attribute (ii) a fuzzy set $\{x_i\}$
representing the target object (iii) the set of object groundings
$\{ v_{i}\}$ and (iv) the set of $\{h_i\}$ objecthood parameters.

As above, all target objects for attribute equality are
definites. Thus, we first renormalize the target object vector so that
it represents a probability distribution over target objects
$p = \textsc{renormalize}(x)$.

The \op{query} operator then computes a matrix representing the
degree to which each object fits each concept
$M \in \mathbb{R}^{|\mathcal{A}| \times n}$.

$$M_{[\conc{m},i]} = y_{\conc{m}} \cdot A_{\att{a}} v_i $$

Here, all variables are as in the \op{filter} operator.

We assume that concept values are mutually exclusive for each object
and implement this by applying \textsc{softmax} to the columns of $M$
to derive a new column-normalized matrix $M^\prime$.

We then compute vector of joint probabilities that the each object is
the target object and has the particular concept value. We renormalize
this vector to derive the desired conditional probability distribution
over concept values for the attribute and object
$o= \textsc{renormalize}(p^\intercal M^\prime)$ . \tjo{I don't know if
  this last step is true, but it seems necessary?}


\todo{operators that only appear in outer scope}

\subsubsection{Count}
top level
count takes a fuzzy set and returns the sum (the expected cardinality
of the set

\subsubsection{Intersect}
Takes in two fuzzy sets and component-wise min (and's them together)

\subsubsection{Disjunction}

max of two sets

\subsubsection{Exists}
top-level
single fuzzy set, returns max in the set

\subsubsection{Count greater/less/Equal}
top-level
``
greater takes 2 fuzzy sets, get expected number of elements for both
sets and run the difference through a sigmoid after an affine
transformation.

equal: take absolute value of the difference and then take the
negative of that run through the sigmoid after affine transformation

\subsubsection{QueryAttribute Equality}
top-level 
``do two objects have the same color''

takes in two distributions over objects

give one of them to relate attribute equality get the result of that
fuzzy set and then multiply that by the probability that each one is
the target (expected probability that two objects have the same value
for an attribute).

